Identification of a Local Sample of Gamma-Ray Bursts Consistent with a Magnetar Giant Flare Origin

Cosmological Gamma-Ray Bursts (GRBs) are known to arise from distinct progenitor channels: short GRBs mostly from neutron star mergers and long GRBs from a rare type of core-collapse supernova (CCSN) called collapsars. Highly magnetized neutron stars called magnetars also generate energetic, short-duration gamma-ray transients called Magnetar Giant Flares (MGFs). Three have been observed from the Milky Way and its satellite galaxies and they have long been suspected to contribute a third class of extragalactic GRBs. We report the unambiguous identification of a distinct population of 4 local ($<$5 Mpc) short GRBs, adding GRB 070222 to previously discussed events. While identified solely based on alignment to nearby star-forming galaxies, their rise time and isotropic energy release are independently inconsistent with the larger short GRB population at $>$99.9% confidence. These properties, the host galaxies, and non-detection in gravitational waves all point to an extragalactic MGF origin. Despite the small sample, the inferred volumetric rates for events above $4\times10^{44}$ erg of $R_{MGF}=3.8_{-3.1}^{+4.0}\times10^5$ Gpc$^{-3}$ yr$^{-1}$ place MGFs as the dominant gamma-ray transient detected from extragalactic sources. As previously suggested, these rates imply that some magnetars produce multiple MGFs, providing a source of repeating GRBs. The rates and host galaxies favor common CCSN as key progenitors of magnetars.

==> old.tex <==
\subsection{The GRB Sample}
Our search methodology requires GRBs that are well-localized, with measured duration, and with bolometric fluence (1\,keV-10\,MeV) determined from broadband instruments. We have considered bursts detected in the last three decades, combining the catalogs from \textit{CGRO}-BATSE\cite{fishman1989batse}, KONUS-\textit{Wind}\cite{aptekar1995konus}, \textit{Swift}-BAT\cite{Barthelmy05}, and \textit{Fermi}-GBM\cite{Meegan09} with the IPN localization information\footnote{ssl.berkeley.edu/ipn3/index.html}. The separate triggers were matched to events utilizing temporal information for all events and spatial information\cite{ashton2018coincident} when available. The considered duration ($T_{90}$) is the shortest value reported by any individual catalog. The total sample contains more than 11,000 GRBs observed, with $>$1,200 GRBs using the standard 2\,s cutoff. 

The bolometric (1\,keV-10\,MeV) fluence is not a standard entry in any input catalog. We convert fluence values measured by broadband instruments from instrument-specific measurement ranges to the bolometric range when spectral parameters are known. Otherwise we scale the reported fluence by the median of the instrument-specific fluence to the bolometric fluence. Intercalibration uncertainties are within $25\%$. 

\textit{CGRO}-BATSE observed GRBs from Low Earth Orbit between 1991 and 2000. The trigger and location information are from BATSE 4B Catalog\cite{paciesas1999fourth}. The spectral catalog values are from the BATSE 5B Spectral Catalog\cite{goldstein2013batse}. The Spectral Catalog reports fluence in the 20-2000\,keV energy range. We apply the largest BATSE localization systematic error\cite{briggs1999error} to our sample, giving quasi-circular localizations of $\sim$5-10\,deg accuracy (uncertainties in this section are quoted at 1-sigma).

Konus-\textit{Wind} has observed short GRBs from the L1 Lagrange point since its launch in 1994. The KONUS spectral information comes from the published short GRB catalog\cite{svinkin2016second} with more recent values taken from GCN Circulars or performed for this work. These are guided by the preliminary list of KONUS short GRBs after the prior catalog\footnote{\url{http://www.ioffe.ru/LEA/shortGRBs/Current/index.html}}. KONUS localizations are an ecliptic band with typical $\sim$10\,deg uncertainty.

\textit{Swift} has observed more than 100 short GRBs since its launch in 2004 to Low Earth Orbit. BAT is the prompt GRB monitor which provides localizations at $\sim$arcminute accuracy, but does not have broadband energy coverage. Therefore, we utilize its location and duration information, but require an external fluence measurement. Values are from the \textit{Swift}-BAT Catalog\cite{Lien2016third}, which is periodically updated online\footnote{\url{https://swift.gsfc.nasa.gov/results/batgrbcat/index.html}}. More recent BAT observations and \textit{Swift} X-ray Telescope localizations (used when available) are from the unofficial \textit{Swift} GRB Table\footnote{\url{https://swift.gsfc.nasa.gov/archive/grb_table/}}.

\textit{Fermi}-GBM has observed GRBs from Low Earth Orbit since its launch in 2008. The spectral and temporal parameter measures for \textit{Fermi} GBM are from the published catalogs\cite{von2020fourth}. We have generated GBM localization skymaps using the latest methods\cite{goldstein2020evaluation} for all bursts.

The IPN compiles localization information for GRBs, including the timing annuli derived from the relative arrival times of gamma-rays at distant spacecraft. Information used here is from the IPN localizations of Konus short GRBs through 2020\cite{pal2013interplanetary} and the IPN list kept up to date online\footnote{\url{http://www.ssl.berkeley.edu/ipn3/}}. Additional IPN localizations were compiled for more than 100 additional short GRBs for this work, which were added to the online table. %GRB\,070222 was originally identified by our search as a marginally interesting candidate based on information from a single annulus. In investigating this as a candidate MGF it was discovered that INTEGRAL also detected the burst, allowing for an additional annulus used here.

All of the location information from the autonomous localizations (i.e. GBM, BATSE, Swift, KONUS), timing annuli (instrument pairs), and Earth occultation selections are converted to the HEALpix\cite{gorski2005healpix} format using the GBM Data Tools\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/gbm/gbm_data_tools/gdt-docs/}}. Systematics are included for GBM and BATSE localizations and IPN annuli. We utilize symmetric annuli uncertainties, using the conservative value from asymmetric measures. The final combined localizations are from renormalizing the product of the independent PDFs.

The localization threshold is set to a 90\% confidence area $<4.125$\,deg$^2$ when including systematic error. This value is chosen as it is 1/10,000 the area of the sky, it is comparable to the total angular size on the sky of galaxies within 200\,Mpc ($\sim$2\,deg), and it is between previously used thresholds\cite{GMF_IPN_Dmitry_search}. With the bolometric fluence measure requirement and the removal of bursts with known redshift\cite{Lien2016} beyond the distance where the event may be a detected MGF, we are left with a sample of 250 short GRBs.

==> old_version_copy.tex <==


\textbf{The two known progenitors of GRBs are collapsars and neutron star mergers both of which have been confirmed with 'smoking-gun' signatures. Collapsars power long GRBs and subsequent broad-lined type Ic supernovae\cite{galama1998unusual,cano2017observer}. Neutron star mergers first produce a loud gravitational-wave chirp signal and then power the short GRB as directly confirmed with GW170817 and GRB 170817A\cite{GW170817-GRB170817A}. 

Neither of these progenitors could have powered our sample of local events. The prompt GRB duration is inconsistent with a collapsar scenario and no supernovae were reported in the galaxies following the GRBs\cite{li2011nearbyii}. LIGO non-detections in gravitational waves exclude this origin for three of the four events\cite{abbott2008implications,abadie2012implications,aasi2014search}, but are insufficiently sensitive to inform on the origin of GRB\,200415A. We have therefore achieved discovery significance for a new progenitor class of GRBs. These bursts are 4 out of our full sample of 250 GRBs, corresponding to $\sim$2\% of detected short GRBs, or $\sim$0.3\% of all GRBs (as long GRBs are detected more often). Lastly, these four bursts are the closest known by an order of magnitude.}

\textbf{We now investigate what caused these 4 bursts. There are 'smoking-gun' signatures of MGFs, but these are not detectable to extragalactic distances with current facilities. To investigate the origin of these events we follow the prescription that tied most short GRBs to neutron star mergers prior to GW170817 and GRB 170817A, which included the lack of detected supernova following the GRB for nearby events (confirmed above), the favoring of older progenitors through the association to early-type host galaxies, and the position of the GRB relative to the host\cite{fong2015decade}. MGFS originate from young magnetars, which are generally believed to be remnants from the deaths of massive stars. Then, MGFs would arise in star-forming galaxies or star-forming regions. Within our maximal detection distance the galaxies with the highest SFR are M82, M83, NGC\,253, and NGC\,4945\cite{mattila2012core}. GRB 051103 is associated to M82 by our method and in a region with known star-forming knots\cite{ofek2006short}, GRB 070222 to M83, and GRB 200415A to the star-forming core of NGC\,253\cite{IPN2020}. GRB 790305B is associated to the star-forming Large Magellanic Cloud. Thus, following field-standard methodology we favor an MGF origin for these events.}

\textbf{We have an advantage over the studies investigating a neutron star merger origin for most short GRBs: we can compare their properties to those expected based on observations of the 3 known MGFs. To investigate an MGF origin we compare values of two key prompt emission parameters}, plotted together in Figure\,\ref{fig:FAR} but considered separately for classification (Methods). First, MGFs have rise times of order a few ms, far shorter than most cosmological short GRBs\cite{hakkila2018properties}. We compare values of Time to Peak, the time from the beginning of significant GRB emission to the peak counts interval. An Anderson-Darling k-sample test rejects the null hypothesis that these four are consistent with our bright short GRB sample at $>$99.9\% ($>$3$\sigma$) confidence. Second, MGF $E_{\rm iso}$ values are orders of magnitude fainter than cosmological GRBs, where only the unusual GRB\,170817A\cite{GW170817-GRB170817A} is comparable. Using the same test on this parameter the null hypothesis is again rejected at $>$99.9\% confidence. The four bursts are consistent with the parameter values of the known MGFs.

Three of the four are discussed in the literature. GRBs\,200415A and 051103 are the most robust identifications of extragalactic MGFs based on our significance assessment and the results of partner analyses \textbf{including lightcurve morphology and sub-millisecond variation of the prompt emission}\cite{IPN2020,GBM2020}. GRB\,070201 has the least robust MGF classification; however, the localization is comparatively large ($\sim$x10 the other events) and M31 has the largest angular size of any galaxy in our sample, together lowering $\Omega$ even for real associations. We confirm this by checking GRB\,790305B with the Large Magellanic Cloud, which has even larger angular extent than M31, giving $\Omega=500$. Last is the newly identified GRB\,070222 which is in-class with the key properties of MGFs (Extended Data Table 1) but \textbf{suggests MGF events can have multiple pulses}, as shown in Figure\,\ref{fig:lc}.

\textbf{To summarize the observational case for an MGF origin: these events localize to the nearby universe and in particular to star-forming regions or star-forming galaxies. The prompt emission is inconsistent with a collapsar origin and gravitational wave observations exclude a compact merger involving neutron stars and/or black holes. The event rates, quantified below, are in excess of the majority of energetic astrophysical transients but are consistent with predictions from the known MGFs. The properties of the prompt emission is distinct from the larger short GRB population but again consistent with the properties from the known MGFs. There is additional evidence for individual events in partner analyses. We conclude that we have confirmed a sample of extragalatic MGFs that match prior predictions on detection rates and properties from both theoretical and observational studies.}

A remaining question is: why have we not identified MGFs at greater distances? Based on previous knowledge MGFs were thought to be detectable to tens of Mpc. The spectra of the initial pulse of GRBs\,200415A, 051103 (Extended Data Table 1), and GRB\,070222 (Supplemental Material) are particularly spectrally hard with shallow spectral index and high peak energies, which is consistent for GRB\,041227\cite{GMF_041227_SGR1806_Frederiks}. Such a spectrum, compared to a typical short GRB, would have only 15-20\% of the photons in a nominal triggering energy range. As GRB monitors are triggered by photon counts, this reduces the effective detection volume to the most luminous MGFs by a factor $\sim$100. \textbf{Further, there is a local overdensity within $\sim$5\,Mpc of CCSN\cite{mattila2012core}, which explains the excess of detections within this range and lack of detections beyond it.}

\textbf{Under the assumption of an MGF origin, we can place new constraints on the properties of MGFs and the formation channel of magnetars.}
With our full MGF sample we constrain the intrinsic energetics function and volumetric rates (Methods). Considering the known energetics range, with an assumed power-law form we measure $\alpha=1.7\pm0.4$ at 90\% confidence. Considering the dominant sources of uncertainty, we infer a volumetric rate of $R_{MGF}=3.8_{-3.1}^{+4.0}\times10^5$\,MGFs\,Gpc$^{-3}$\,yr$^{-1}$, orders of magnitude above the volumetric rates of cosmological GRBs\cite{siegel2019collapsars}.



Magnetars may be generated in a variety of events including common CCSN, low-mass mergers\cite{2006Sci...312..719P}, a rare evolution of white dwarfs\cite{2007ApJ...669..585D}, or a rare sub-type of CCSN such as collapsars or superluminous supernovae\cite{nicholl2017magnetar}. Each of these is consistent with the observed association of magnetars to supernova remnants\cite{beniamini2019formation}. Low-mass merger events have long inspiral times and should track total stellar mass rather than the current SFR, inconsistent with our sample. A CCSN origin would arise from regions with high rates of star formation. This is consistent with our observations and bolstered by both the lack of detections beyond 5\,Mpc due to the local SFR overdensity and the detection of GRB\,790305B from the low-mass, star-forming Large Magellanic Cloud. The host galaxies of our extragalactic sample and the Milky Way itself have larger mass and higher metallicity than is typically seen in hosts of collapsars or superluminous supernovae\cite{2019arXiv191109112T}. Therefore, the types of host galaxies favor common CCSN as the dominant formation channel of magnetars.

Additional support for this conclusion is provided from the rates of these events. We can relate our inferred MGF rates to progenitor formation rates\cite{tendulkar2016radio} as $R_{MGF} = R_{Event} f_M \tau_{Active} r_{MGF/M}$ where $R_{Event}$ is the rate of events that may form magnetars, $f_M$ is the fraction that successfully form magnetars, $\tau_{Active}$ the timescale that magnetars can produce MGFs, and $r_{MGF/M}$ the rate of MGFs per magnetar. We take $\tau_{Active} \approx 10^4$\,yr limited by the decay of the magnetic field\cite{beniamini2019formation}. Given the incompleteness of our known magnetar sample and lack of understanding which magnetars can produce MGFs, we use the 3 known to be capable to place an upper bound of $r_{MGF/M}<0.02$\,MGFs\,yr$^{-1}$ per magnetar.

Of the discussed formation channels only CCSN are both expected to track star-forming regions and have a comparable volumetric rate, being 7$\times10^4$\,Gpc$^{-3}$\,yr$^{-1}$ in the local universe\cite{li2011nearby}. A fiducial value on $f_M$ is 0.4 with a 2$\sigma$ confidence interval of 0.12-1.0\cite{beniamini2019formation}. Then, we require either that some magnetars produce multiple MGFs or that both $f_M\approx1$ and the true rate of $R_{MGF}$ is near our 95\% lower bound. Using the CCSN rate and the 95\% lower limit on $R_{MGF}$ we can observationally constrain $f_M>0.005$, further excluding particularly rare sub-types of, and favoring common, CCSN as the dominant formation channel of magnetars.

Our analysis suggests additional extragalactic MGFs may be identified with improved analysis and collaboration. \textbf{'Smoking-gun' confirmation likely requires future instruments.} The inferred rates are sufficiently high that they may contribute to the stochastic background of gravitational waves. This, and the recent observations of fast radio bursts associated to lower-energy gamma-ray flares from magnetars\cite{bochenek2020fast}, suggest the coming years will bring new insights into the physics and emission of magnetars. 


% \end{doublespace}

\bibliographystyle{naturemag}
\bibliography{bibliography}


% \pagebreak





























































\begin{figure}[h]
    \centering
    \includegraphics[width=8.9cm]{MGF_rates.png}
    \caption*{\textbf{Methods Figure 3:} The inferred MGF rates as a function of $\alpha$ and N MGFs. The 90\% confidence contour from the combined 2D PDF of these parameters is outlined in white.}
    \label{fig:MGF_rates}
\end{figure}


